2FHL: The Second Catalog of Hard Fermi-LAT Sources

We present a catalog of sources detected above 50 GeV by the {\it Fermi}-Large Area Telescope (LAT) in 80 months of data. The newly delivered Pass 8 event-level analysis allows the detection and characterization of sources in the 50 GeV--2 TeV energy range. In this energy band, {\it Fermi}-LAT has detected 360 sources, which constitute the second catalog of hard {\it Fermi}-LAT sources (2FHL). The improved angular resolution enables the precise localization of point sources ($\sim$1.7$'$ radius at 68 % C.~L.) and the detection and characterization of spatially extended sources. We find that 86 % of the sources can be associated with counterparts at other wavelengths, of which the majority (75 %) are active galactic nuclei and the rest (11 %) are Galactic sources. Only 25 % of the 2FHL sources have been previously detected by Cherenkov telescopes, implying that the 2FHL provides a reservoir of candidates to be followed up at very high energies. This work closes the energy gap between the observations performed at GeV energies by {\it Fermi}-LAT on orbit and the observations performed at higher energies by Cherenkov telescopes from the ground.

==> tab_likelihood.tex <==
\begin{deluxetable}{lccc}
\setlength{\tabcolsep}{0.04in}
\tablewidth{0pt}
\tabletypesize{\scriptsize}
\tablecaption{Likelihood-ratio parametrization \label{tbl-ab}}
\tablehead{
\colhead{$~$} & 
\colhead{NVSS} & 
\colhead{SUMSS} & 
\colhead{RASS} 
}
\startdata
LR$_c$ & 1.57 & 0.29 &2.57 \\
\enddata
\end{deluxetable}

